LLM Code Customization with Visual Results: A Benchmark on TikZ

With the rise of AI-based code generation, customizing existing code out of natural language instructions to modify visual results -such as figures or images -has become possible, promising to reduce the need for deep programming expertise. However, even experienced developers can struggle with this task, as it requires identifying relevant code regions (feature location), generating valid code variants, and ensuring the modifications reliably align with user intent. In this paper, we introduce vTikZ, the first benchmark designed to evaluate the ability of Large Language Models (LLMs) to customize code while preserving coherent visual outcomes. Our benchmark consists of carefully curated vTikZ editing scenarios, parameterized ground truths, and a reviewing tool that leverages visual feedback to assess correctness. Empirical evaluation with stateof-the-art LLMs shows that existing solutions struggle to reliably modify code in alignment with visual intent, highlighting a gap in current AI-assisted code editing approaches. We argue that vTikZ opens new research directions for integrating LLMs with visual feedback mechanisms to improve code customization tasks in various domains beyond TikZ, including image processing, art creation, Web design, and 3D modeling.

==> Metrics_def.tex <==
We present a comprehensive suite of evaluation metrics for assessing predictions. All metrics are normalized to return scores in the range [0,100], where 100 represents perfect alignment with the reference and 0 represents maximum divergence.
\subsubsection{Code-Based Metrics}
Code similarity evaluation is performed using two distinct approaches: full-code evaluation and patch-specific evaluation.

\textbf{BLEU Score} evaluates n-gram overlap (up to 8-grams) between predictions and reference solutions using SacreBLEU's implementation\cite{post_call_2018}, providing a measure of code similarity based on token sequences(using the default mteval-v13a tokenizer).

\textbf{CHRF} (Character n-gram F-score\cite{popovic_chrf_2015}) provides character-level similarity assessment, using a maximum character n-gram order of 6.

\textbf{TER} (Translation Edit Rate) measures the minimum number of edits required to transform the prediction into the reference. The scores are inverted and normalized to maintain consistency with other metrics where higher values indicate better performance.

\textbf{EED} (Extended Edit Distance) implements an extension of the edit distance metric, adding the idea of jumps, a way to move between characters or
blocks \cite{stanchev_eed_2019}.

\textbf{Crystal BLEU} enhances standard BLEU scoring by incorporating awareness from the full corpus of input TikZ code. Essentially removing the 500 most common words from the evaluation of the BLEU metric\cite{eghbali_crystalbleu_2023}.

\textbf{Patch Accuracy} provides a binary evaluation (0 or 100) of exact patch matches, offering a strict assessment of patch correctness.

\textbf{Line-Metric}, this metric is defines as the percentage of correct lines edited, defined as \[
\text{Line-Metric} = \frac{\text{Number of lines edited that are the same}}{\text{Number of lines edited by the solution}}
\]

\textbf{BLEU Patch}, \textbf{CHRF Patch} and \textbf{Crystal BLEU Patch} apply their respective algorithms specifically to patches rather than complete code.

\subsubsection{Image-Based Metrics}
Image evaluation employs diverse metrics to assess similarities via pixel-based and structural approaches:

\textbf{CLIP-Based Evaluation} \cite{radford_learning_2021} utilizes two approaches:
\label{def:clipeval}
Text-to-Image and Image-to-Image similarity, both based on cosine similarity. The first approach measures the similarity between the generated image and a description text (see \cref{sec:dataset_format}), while the second compares the generated image with the reference image. This evaluation uses the open-CLIP model ViT-bigG-14-quickgelu.

\textbf{Feature Matching} employs SIFT\cite{lowe_distinctive_2004} (Scale-Invariant Feature Transform)  to find matching features. Scores are normalized based on the maximum possible matches with the reference image.

\textbf{MSE} (Mean Squared Error) provides a fundamental pixel-level comparison, converted to a similarity score through inverse transformation

\textbf{PSNR} (Peak Signal-to-Noise Ratio) measures the ratio between maximum possible pixel value and distortion, offering a logarithmic scale assessment of pixel fidelity

\textbf{LPIPS} (Learned Perceptual Image Patch Similarity) leverages an AlexNet backbone to assess similarities in a learned feature space, better aligned with human perception

\textbf{MS-SSIM} (Multi-Scale Structural Similarity Index) analyzes structural information preservation across multiple scales, capturing similarities in luminance, contrast, and structure.

\TODO{Cite for each remaining metrics : PSNR, LPIPS }

==> former/analysis.tex <==
\subsection{Valid Variants}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/RQ_diagrams/pass_rate.png}
    \caption{
        Average Percentage of Valid variants for each configuration.
    }
    \label{fig:var_valid}
\end{figure}

\cref{fig:var_valid} shows that the models generate valid variants at least 76\% of the time on average. At pass@1, the worst performing model is the smaller one llama3.1-8b, and the best performing one is DeepSeek-R1-Distill-Llama-70B. Increasing the temperature and the pass@k to 5 with this best performing model reduced the average performance by 10\%, whereas with the llama 3.3 model, it \TODO{Add the new results}

Nevertheless, at pass@1, with the same temperature, the reasoning model generates valid variants 96\% of the time compared do its non-reasoning counterpart, achieving 90\%.
\conclusion{%
Findings: At pass@1 with a temperature at 0.7, the latest models generate valid variants on average at least 90\% of the time, and up to 96\% for the reasoning model. Our experiment also shows substandard but correct results on models that can run on consumer hardware, with llama-3.1-8b achieving a valid variant on average 76\% of the time.
}
\subsection{Sound Variants}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/RQ_diagrams/irght_lines_measures.png}
    \caption{
        Average Percentage of Correct Lines Edited for Each Configuration.
    }
    \label{fig:var_sound}
\end{figure}

Our measurements, displayed in \cref{fig:var_sound}, shows underwhelming results overall, with models editing on average at most 43\% of the correct lines. Unlike the previous results, the reasoning model did not achieve better results than its non-reasoning version, both respectively achieving 43\% and 42.7\%.

This time, at pass@5, the two evaluations of the model DeepSeek-R1-Distill-Llama-70B at two different temperature achieved extremely similar results. Even though more "random" output would theoretically augment the chances to edit the right lines, its also augment the chances of generating non-valid variants, resulting in similar performances overall when it comes to \emph{Sound} variants.
\TODO{Compare with the results of llama pk5 t1.5}

\conclusion{%
\textbf{RQ2: In the current state, LLMs and MLLM\TODO{Maybe statement not true, depend on the evaluation with multimodal} fail to identify the correct features, leading to poor results in generating sound variants. Potentially highlighting a fundamental limitation in the capabilities of all SOTA models.} 
}

\subsection{Perfect Variants}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/RQ_diagrams/same_patch_measures.png}
    \caption{
        Average Percentage of Perfect Variants for Each Configuration.
    }
    \label{fig:var_perfect}
\end{figure}

As shown in \cref{fig:var_perfect}, all of the model achieved poor performances. The reasoning model achieved slightly better results than the rest of the models, while the Llama 3.0 and 3.3 70b models did not generate any perfect variants. Even thought these variants can't be considered as the only ones achieving a good results, these measures still show a lack of performances in their general ability. 
\conclusion{%
\textbf{RQ3: In all evaluated models, the generated variants rarely match the theoretically perfect ones. Given the precision required by some edits, these findings highlight the need for improved approaches that more accurately capture and apply the underlying intent of edits.} 
}

\subsection{Correct Variants}

==> former/analysis_2.tex <==
\subsection{"Formal" Metrics}
\begin{table}
    \centering
    \input{Tables/Metrics/avg_by_config_patch_line}
    \caption{
         "Formal" Metrics achieved by the models evaluated(in percentages).
    }
    \label{tab:metric_formal}
\end{table}


The averages of \emph{LineMetric}, \emph{PatchMetic}, and the number of valid variants for each configuration are given concatenated in \cref{tab:metric_formal}. As described above, it can happen that the model does not follow the instructions of generating between back-ticks, in that case, the variants concerned are ignored from the computations of the metrics(hence the 8.1 score of distill-llama on the PatchMetric).

\paragraph{Averages of formal metrics}
In \cref{tab:metric_formal}, it first stands out that only approximately 9 out of 10 generated variants are valid, showing a first flaw in using LLM to generate TikZ Code. Secondly, the models rarely edit the right lines, with at most 49.2\% of the time on average by llama3.3-70b. Interestingly, the distilled version of this model performs worse by editing the right lines only 41.3\% of the time, though it does achieve better performances in finding the exact patch.\\
Overall, we do find an upward trend in their performance in relation to their number of parameters and release date.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/RQ_diagrams/concentric_variant_classif.png}
    \caption{
        Number of variants in each category.
        }
    \label{fig:var_classif}
\end{figure}
\paragraph{Number of variants}
The \cref{fig:var_classif} gives an overview of the number of variants in each category. As seen in these results, the distill-llama reasoning model achieves better performances in finding \emph{Perfect} variants, but does not generate as much \emph{Sound} variants as its non-reasoning counterpart, which only achieves 42 out of 100.\\
In spite of being state-of-the-art models, \cref{fig:var_classif} already points at a deep flaw in these LLMs, that can hardly be trusted, even when only considering \textit{Valid} variants.



\subsection{State of the Art Metrics}
In this section, we explore the measurements of several State of the Art Text-based and Image-based metrics on the variant generated.

\begin{table}
    \centering
    \input{Tables/Metrics/avg_by_config_full_text}
    \caption{
         Full Text Based Metrics achieved by the models evaluated(in percentages).
    }
    \label{tab:metric_fulltext}
\end{table}

\begin{table}
    \centering
    \input{Tables/Metrics/avg_by_config_patchtext}
    \caption{
         Patch based Text Metrics achieved by the models evaluated(in percentages).
    }
    \label{tab:metric_patchtext}
\end{table}

\paragraph{Text-based metrics}
The \cref{tab:metric_fulltext} displays the metrics computed on the entirety of the codes, comparing the perfect variants with the variants generated, as the generated and original files are mostly the same, the achieved scores are higher and exhibit very little variation, with at most a difference around 5 with the CrystalBleu Metric.
Within these metrics, llama3.3-70 is considered to be the best model, with mixtral-8*7b and llama3.1-8b performing the worse. Because Chrf is based on character comparisons, it does show surprising results, when ranking the distill-llama model as the second to last performing model where the other metrics ones ranks it second. 

The \cref{tab:metric_patchtext} only considers the patches when comparing the variants, comparing only patches yields a much wider variance and meaningful results, especially in the case of Chrf. They display a much uniform ranking overall, with significant difference between each of them.


\begin{table}
    \centering
    \input{Tables/Metrics/avg_by_config_image}
    \caption{
         Image Based Metrics achieved by the models evaluated(in percentages).
    }
    \label{tab:metric_image}
\end{table}
\paragraph{Image-based metrics}
The output images being mostly similar, the image based metrics suffer from the same problem as the full-text metrics. Interestingly however, the ranking is uniform between all but the ClipText Metric, and they rank the deepseek model as the best performing one. 
Our interpretation is that either the text-based metrics are insufficient to clearly identify the best variants, or the image-based metrics do not perform well enough for 2D TikZ diagrams.\\
We explore this question in the following section, by validating the metrics against human preferences. 
